RAIL: Reachability-Aided Imitation Learning for Safe Policy Execution

Imitation learning (IL) has shown great success in learning complex robot manipulation tasks. However, there remains a need for practical safety methods to justify widespread deployment. In particular, it is important to certify that a system obeys hard constraints on unsafe behavior in settings when it is unacceptable to design a tradeoff between performance and safety via tuning the policy (i.e. soft constraints). This leads to the question, how does enforcing hard constraints impact the performance (meaning safely completing tasks) of an IL policy? To answer this question, this paper builds a reachability-based safety filter to enforce hard constraints on IL, which we call Reachability-Aided Imitation Learning (RAIL). Through evaluations with state-of-the-art IL policies in mobile robots and manipulation tasks, we make two key findings. First, the highest-performing policies are sometimes only so because they frequently violate constraints, and significantly lose performance under hard constraints. Second, surprisingly, hard constraints on the lower-performing policies can occasionally increase their ability to perform tasks safely. Finally, hardware evaluation confirms the method can operate in real time.

==> sections/A_meeting_notes.tex <==
\section{Meeting Notes}

\subsection{July $10^{th}$ 2024}{
\subsubsection{Meeting Summary}
\begin{itemize}
    \item \textbf{Progress of the week} 1) The ranking system is implemented to reduce the number of safety interventions.
    2) Safety-filter with diffuser-style policy implemented.
    \item \textbf{Safety intervention}. It significantly reduced the number of safety interventions in the sake of computation time.
    A possible next step is to train a neural network to predict the ranking.
    The inconsistency problem spotted in the previous week is still present and is exacerbated in some sense, leading to the performance degradation of the safety filter with ranking.
    \item \textbf{Correct choice of the state prediction model}. 
    The proposed diffusion plan is separated into the head plan, which is analyzed for safety, and the tail plan, employed for guiding the safety filter as the projection objective function. 
    The maze 2D example inspires that the dynamics are not necessarily the correct way to capture the state-action correspondence.
    So, the correct way is to let the dynamics take charge of the safety, and the state distribution model take charge of the performance.
    The initial result of diffuser state prediction is not good.
    \danfei{Adding notes - Danfei suggested using the state-distribution model for both our safety and performance purposes and padding the obstacles with a certain margin for safety purposes.}
    \item \textbf{Next Step: }
    We have two options for the next step, 1) training a model to predict the ranking, and use guiding or ranking, and 2) coming back to the manipulation setting and implementing what we have figured out in the pick-and-place setting.
    It would depend on what story to tell at ICRA, and I should discuss this further with Shreyas based on the discussion with Danfei today.
\end{itemize}
}

\subsection{July $5^{th}$ 2024}{
\subsubsection{Meeting Summary}
\begin{itemize}
    \item \textbf{Progress of the week.} Switching safety filter implemented in Maze 2D environment.
    \item \textbf{Consistency of the diffusion model}
    One interesting problem observed in Maze 2D environments is inconsistent action generations of the diffusion model and its impact on the performance of the safety filter, which is hypothesized to be attributed to the sub-optimality of the Offline RL dataset.
    In those cases, projecting the diffusion plan results in undesired behavior as oscillating, and equipping the safety filter with its performance metric (e.g., goal mode) resolved the inconsistency.
    However, this kind of strategy is not universal since defining a goal state is not obvious in some tasks (e.g., flipping a mug cup.)
    This reveals one ideal property of a safety filter with a learning method: sensing the learning-based policy's abnormality and recovering the state to where policy can generate consistent actions (or in-distribution state).
    This is beneficial to choosing an expressive parameterized planner.
    This leads to the following question:
    \textit{Can we make a safety filter to recover to the in-distribution state?}
    \item \textbf{Frequent interventions}
    We observe frequent safety interventions in Maze 2D examples.
    In the worst case, 80 percent of the actions are suggested by the backup planners, not diffusion planners.
    This is possibly attributed to the Offline RL dataset where velocity lies in [-5, 5] and high-velocity policy might be adversarial to computing the backup plan in such a cramped environment like Maze where we have free space of 1 $m$.
    This, in turn, leads to the following question: \textit{Can we make a diffusion plan to propose the plan that minimizes the safety intervention?}
\end{itemize}
}

\subsection{Jun $21^{th}$ 2024}{
\subsubsection{Meeting Summary}
\begin{itemize}
    \item Diffusion policy implemented on Maze-2D in robomimic environment.
    \item \textbf{Local trap problem and solutions:} The diffusion policy with a safety filter suffers from the problem where the robot is locally trapped.
    This is hypothesized to happen because the backup plan projects the diffusion policy, possibly causing two problems: 1) the robot might go to the state out-of-distribution (Nearest Neighbor), and 2) the robot remains in the region in a state region where the diffusion policy keeps generating the unsafe policy.
    Two suggested solutions are 1) projecting back to the in-distribution data regime, 2) backup policy exploring, intending to get out of the local trap.
    \item \textbf{Discussion about the minimal model for safety context}: Diffusion policy is powerful since it is model-free.
    However, the safety filter needs an analyzable model.
    Maybe all we need is the minimal model, that is required for the safety-context.
    We can start with the task where this definition is readily available but complicated enough.
    \item \textbf{Week of the goal}: 1) Build a simple safety filter for Maze-2D example in Mujoco environment, 2) Train diffusion policy that predicts the state. 3) The stretch goal is guiding diffusion policy using the safety filter.
\end{itemize}
\subsubsection{Logging thoughts}{
\begin{itemize}
    \item \textbf{Proper Pair of Diffusion Planner and Safety Filter}:
    \textit{By and large, the framework can be interpreted as diffusion policy learns the \textit{target distribution}, the plan becomes \textit{sampling from this distribution}, and the safety filter is filtering this sample to be the executable format for the robot}.
    Hence, we have to choose the \textbf{target distribution} of the diffusion policy, how do we \textbf{plan-ify} the sample from the distribution, how does safety-filter 

    
    The diffusion planner can be largely divided into three categories based on the target distribution of modeling: 1) joint distribution of state and actions \cite{janner2022planning}, 2) state distribution \cite{ajay2022conditional}, 3) action distribution \cite{chi2023diffusion}.
    Now, the diffusion planner follows Diffusion-Policy style \cite{chi2023diffusion} where the policy outputs a sequence of actions conditioned on the high-dimensional states.
    This is advantageous in such a scenario where states are better posed as raw sensor input (e.g., image) since predicting a sequence of states might cause additional problems such as training stability and computation time in Diffuser-style \cite{janner2022planning} planning.

    However, many safety filters require an analyzable model and state, since the safety inherently grounds on how we define the state, not actions.

    Then, it boils down to the following central question: \textit{Can we build a simple model only for the safety context}?
    This model needs not to capture the comprehensive context of the environment but rather focus on \textit{modelable yet safety-critical} context.
    This relies on the assumption that modeling safety-related context is much simpler than modeling comprehensive context.
    For example, when chopping onion, the models we need for a safe backup policy are much simpler; it does not have to interact with the onion - just retract and stop so that the knife does not cut anything.
    
    \wonsuhk{}
    Especially, RTD-style is good at reach-avoid tasks specified by "start $x_0$, end $x_g$, do not hit $O$".
\end{itemize}
}

\subsection{Apr 24th 2024}{
\subsubsection{Meeting Summary}{
\begin{itemize}
    \item I would come up with the idea to orient the Safe Diffusion project and Neural PARC project into a common base. (e.g., can we use Neural PARC as a safety filter of diffusion policy, or can we just use diffusion policy to propose a goal.)

    \item Both agreed that focus should be on diffusion project rather than Neural PARC.

    \item To identify the contribution of the safety-filter idea, read three papers that Shreyas suggested \cite{althoff2019effortless, selim2022safe, thumm2022provably}
\end{itemize}
}

\subsection{Mar 29th 2024}{
\subsubsection{Meeting Summary}{
\begin{itemize}
    \item Matt would work on training diffusion policy that predicts the end-effector position and orientation in robomimic with Kinova Gen-3.
    \item I would convert the end-effector position to joint angle using inverse kinematics and then run safety a filter over there.
    
    
\end{itemize}
}




\subsection{Mar 27th 2024}{
\subsubsection{Meeting Summary}{
\begin{itemize}
    \item Completed implementing the working pipeline of safety filters in Python. 
    A head-plan safety check is checking the intersection of forward occupancy and obstacles at discrete times.
    A backup-plan safety check is implementing the safety layer that uses ARMTD with a cost function that minimizes the gap between configuration path errors.
\end{itemize}
\subsubsection{TODO}{
\begin{itemize}
    \item Improve the head-plan safety check to the intersection of forward occupancy and obstacles at \textbf{a continuous time}.
    Implement two approaches: 1) zonotopic JRS (enclose $cos-sin$ with zonotopes), and 2) polynomial zonotopic JRS (model time interval and use polynomial zonotope arithmetic.)

    \item If Matt finishes setting up the environment (robomimic pick-and-place task and diffusion policy trained on Kinova Gen-3), move every codes to that environment.

    \item Write the chronological plan to improve each module before submitting this to CoRL.
    
    
\end{itemize}
}

==> sections/old_introduction.tex <==
\section{Introduction} \label{sec:intro}
\textbf{Diffusion models have shown great success including the robotics domain.}
Diffusion models have shown great success in generating high-dimensional data such as image, video, and audio.
Recently, the diffusion model has been actively explored in the domain of robotics as reinforcement learning \cite{janner2022planning, ajay2022conditional}, imitation learning \cite{chi2023diffusion, mishra2023generative}, and trajectory generation \cite{carvalho2022conditioned, power2023sampling, carvalho2023motion}. 

\wonsuhk{Review of the pros and cons of using diffusion models in motion planning.}
\textbf{Diffusion models can flexibly synthesize behavior and constraints, but without safety guarantee and low generation speed.}
The notable merit of diffusion policy is its ability to represent multi-modal policy and its runtime controllability.
Despite its appealing traits, its lack of a guarantee of hard constraint satisfaction makes it not favored for safety-critical applications.
Only a few works have explored this area \cite{xiao2023safediffuser}.

\wonsuhk{Review of literature using safety-guided diffusion policy for motion planning.}
\textbf{There exists a research thread that safety constraints guide the diffusion model, which fails to provide neither theoretical nor empirical guarantee as we will see in Section \ref{sec:results}.
}
One research line is to inform the diffusion models of safety constraints by leveraging conditional generation using classifier-guidance diffusion \cite{dhariwal2021diffusion} and classifier-free diffusion \cite{ho2022classifier}.
They achieve this by designing trajectory-wise cost function that penalizes safety violation  \cite{janner2022planning, ajay2022conditional, carvalho2022conditioned} or training classifier \cite{carvalho2023motion} that tells whether the trajectory is safe or not.

\wonsuhk{Review of literature that provably "shields" the generation of the diffusion models}
\textbf{There exists a method that directly interferes with the denoising process to \textit{provably} prevent the generation of unsafe trajectories using invariance \cite{xiao2023safediffuser}.
}

\wonsuhk{Review of safe learning-based control (e.g., safe RL, safety certificate)}
\textbf{Our approach is motivated by safe learning-based control literature, however thanks to the diffusion model's suitability for the long-horizon problem and its controllability, such a method fits more with the diffusion model.}
Before having evidenced the efficiency of diffusion models on planning in the robotics domain, there was a similar effort to guarantee the safety of the action generated by reinforcement learning.

\wonsuhk{Review of safe learning-based control using reachability in specific} \cite{}

\subsubsection*{Contributions}
In this paper, we propose a receding-horizon motion policy that inherits the advantage of the diffusion policy while being provably safe by leveraging parameterized reachability analysis.
Our approach is hierarchical in that it has two motion policies: \textbf{performance policy} modeled as diffusion policy, and overlaying \textbf{safe backup policy} modeled as analyzable, parameterized policy.

% \shrey{
% \begin{outline}
%     \1 First briefly restate the contribution of \textit{this} work
%     \1 Then explain, at a high level, what aspects of the literature our work is related to (e.g., we use diffusion policies and a manipulator safety filter)
%     \1 Your overall goal is to answer the following questions:
%         \2 What have other people done that tries to solve the same or similar problems?
%         \2 What gaps remain from those other methods that we attempt to solve with this paper?
% \end{outline}
% }

% \subsection{Offline Imitation Learning with Diffusion Policy}


% \textbf{Model-free learning has shown great success in the robotics domain.}
% Learning complex behavior policies requires knowledge about the target task, success metrics, environment dynamics, and human supervision. While reinforcement learning provides an effective framework for learning target behaviors, it requires a lot of interactions with the environment in addition to designing a representative reward function. Availability of online human expert demonstrations bypasses the need for a reward function but still requires to interact with the environment. In such a scenario, learning target behaviors from pre-recorded offline demonstrations by imitation has proven promising as it circumvents the need to undergo physical interactions with the environment. For such a paradigm, many recent works have shown impressive generalization \cite{padalkar2023open}, performance \cite{shafiullah2022behavior}, and ability to generate temporally consistent plans~\cite{chi2023diffusion}. In this work, we aim to build on top of effective imitation learning frameworks.

% \textbf{Imitation models can flexibly synthesize behavior and constraints, but without safety guarantees.}
% \utkarsh{also write about compounding error, OOD error and not reactive to changes in the environment at inference and then safety}
% Despite their appeals, one major drawback of robot learning models is the lack of a guarantee of hard constraint satisfaction which makes them unsuitable for safety-critical applications.
% Only a few works have tried to explore this area \cite{xiao2023safediffuser, chen2019deep, yin2021imitation}. Guaranteeing safety for deep-learned policies is challenging due to the black-box nature of these models. Furthermore, slight changes in the environment might introduce covariate shift \cite{bagnell2015imitation} and cause the model to make erroneous predictions. These errors can compound leading to unpredictable and dangerous behavior \cite{}.  Our work attempts to combine the performance and flexibility of deep-learning models, with the safety guarantees of \nadun{conventional robot planning (rephrase this?)}.

==> sections/old_problem.tex <==
% \section{Problem Statement}\label{sec: problem statement}
% \subsubsection*{Problem Formulation}
% \begin{problem}
%     Control a robot using a generative, learned motion policy while ensuring the robot avoids collision with obstacles.
% \end{problem}


% Given a dataset of trajectory $D = \{\tau_i\}_{i=1}^N$ where each trajectory is the sequence of the state and action $(s_t, a_t) \in S \times A$, namely $\tau_i=\{(s_t^{(i)},a_t^{(i)})\}_{t=1}^{T^{(i)}}$.
% The planning horizon is set to be $H \in \N$.
% The diffusion policy is denoted as $f_\theta: S \rightarrow (S \times A)^H$, which models unconditioned probability distribution $p_\theta(\tau)$.
% The parameterized safe motion policy is denoted as $\dot s = f\lbl{plan}(t, s; k)$.
% The closed-loop dynamics of the robot under control policy that tracks the trajectory $\tau$ is denoted as $\dot x = f\lbl{track}(t, x; \tau)$.
% We assume that the system is fully observable.

% \begin{problem}
%     Given an initial state $x_0 \in X$, the goal state $g \in S$, the static obstacles $\mathcal O$, and the diffusion policy $f_\theta$ trained on the dataset $D$, design a motion policy that drives the robot to reach $g$ with a provable guarantee of not colliding with $\mathcal O$ when tracked.
% \end{problem}

==> sections/old_related_work.tex <==
% \subsection{Related Work}
% \shrey{
% \begin{outline}
%     \1 First briefly restate the contribution of \textit{this} work
%     \1 Then explain, at a high level, what aspects of the literature our work is related to (e.g., we use diffusion policies and a manipulator safety filter)
%     \1 Your overall goal is to answer the following questions:
%         \2 What have other people done that tries to solve the same or similar problems?
%         \2 What gaps remain from those other methods that we attempt to solve with this paper?
% \end{outline}
% }

% \subsection{Diffusion Model}
% \subsection{Parameterized Reachability}
% Reachability-based Trajectory Design (RTD) \cite{kousik2017safe} is a receding-horizon, real-time trajectory planner that generates provably safe trajectories. 
% It uses zonotopes as reachable sets to approximate all possible robot positions from a continuum of parameterized trajectories. 
% Note that the reachable sets are constructed such that collision-avoidance is guaranteed in continuous-time. 
% RTD solves a constrained optimization problem to select a feasible trajectory such that the swept volume corresponding to the chosen trajectory is guaranteed to be collision free. 
% For the possibility that a feasible trajectory is not found, a fail-safe maneuver is executed to bring the robot safely to a stop.
% In recent years, there have been extensions of RTD to robotic arms \cite{holmes2020armtd}, \cite{michaux2024safe}, \cite{michaux2023can} which have demonstrated real-time, safe trajectory planning. Our work will utilize \cite{holmes2020armtd} as our backup planner.
% \dennis{Added this in here. May need to reword}

% \shrey{I thnk this paragraph shoudl be merged into the related work}
% Previous attempts to address safety in learned policies have explored various approaches. Some methods integrate IL with safety controllers using safe set theory \cite{chen2019deep}, although primarily in lower-dimensional spaces. Others have proposed informing diffusion models of safety constraints through conditional generation techniques \cite{janner2022planning, ajay2022conditional, carvalho2022conditioned, carvalho2023motion}. However, these approaches often lack theoretical or empirical guarantees on the safety of generated actions. \danfei{Probably need a bit more survey here.}


% \danfei{Need to cover more broadly safety for learned policies here. why they don't work / lack guarantees. then talk about specifically safety for diffusion policies}


% \danfei{Talk about safety filter, why they are great}
% \nadun{Include safety filter stuff below}
